On the validity of many-mode Floquet theory with commensurate frequencies

Many-mode Floquet theory [T.-S. Ho, S.-I. Chu, and J. V. Tietz, Chem. Phys. Lett., v. 96, 464 (1983)] is a technique for solving the time-dependent Schr\"odinger equation in the special case of multiple periodic fields, but its limitations are not well understood. We show that for a Hamiltonian consisting of two time-periodic couplings of commensurate frequencies (integer multiples of a common frequency), many-mode Floquet theory provides a correct expression for unitary time evolution. However, caution must be taken in the interpretation of the eigenvalues and eigenvectors of the corresponding many-mode Floquet Hamiltonian, as only part of its spectrum is directly relevant to time evolution. We give a physical interpretation for the remainder of the spectrum of the Hamiltonian. These results are relevant to the engineering of quantum systems using multiple controllable periodic fields.

==> sections/equation_labels_generated.tex <==
\newlabel{eq:each_floquet_soln}{{1}{1}{}{}{}}
\newlabel{eq:quasi_fourier_expansion}{{2}{1}{}{}{}}
\newlabel{eq:tdse}{{3}{2}{}{}{}}
\newlabel{eq:floquet_operator}{{5}{2}{}{}{}}
\newlabel{eq:general_fa_solution}{{6}{2}{}{}{}}
\newlabel{eq:quasi_components}{{7}{3}{}{}{}}
\newlabel{eq:time_evolving_qs}{{8}{3}{}{}{}}
\newlabel{eq:floquet_hamiltonian}{{10}{3}{}{}{}}
\newlabel{eq:shift_def}{{11}{3}{}{}{}}
\newlabel{eq:shift_properties}{{12}{3}{}{}{}}
\newlabel{eq:shirley_propagator}{{14}{3}{}{}{}}
\newlabel{eq:example_hamiltonian}{{15}{4}{}{}{}}
\newlabel{eq:two_electric_coupling_example}{{17}{4}{}{}{}}
\newlabel{eq:relabel}{{19}{5}{}{}{}}
\newlabel{eq:general_h_fourier_expansion}{{20}{5}{}{}{}}
\newlabel{eq:general_mmft_hamiltonian}{{21}{5}{}{}{}}
\newlabel{eq:mmft_propagator}{{22}{5}{}{}{}}
\newlabel{eq:multiple_solutions}{{23}{6}{}{}{}}
\newlabel{eq:t_f1_f2_def}{{25}{7}{}{}{}}
\newlabel{eq:mmft_hamiltonian_translational_invariance}{{26}{7}{}{}{}}
\newlabel{eq:k_basis_def}{{27}{7}{}{}{}}
\newlabel{eq:this_should_be_an_integral}{{29}{8}{}{}{}}
\newlabel{eq:propagator_with_k_equal_zero}{{30}{8}{}{}{}}
\newlabel{eq:required_matrix_element_equality}{{31}{8}{}{}{}}
\newlabel{eq:h_sft_mmft_correspondence}{{32}{8}{}{}{}}
\newlabel{eq:phases_general_h_fourier_expansion}{{33}{8}{}{}{}}
\newlabel{eq:phases_general_mmft_hamiltonian}{{34}{9}{}{}{}}
\newlabel{eq:k_phase_relationship}{{38}{9}{}{}{}}
\newlabel{eq:n_one}{{A1}{11}{}{}{}}
\newlabel{eq:mmft_propagator_promote_demote}{{B1}{12}{}{}{}}
\newlabel{eq:dp_identity}{{B4}{12}{}{}{}}
\newlabel{eq:powers_of_h_equivalence}{{B6}{12}{}{}{}}
\newlabel{eq:hd_dh}{{B7}{12}{}{}{}}

